Temporally Constrained Neural Networks (TCNN): A framework for semi-supervised video semantic segmentation

A major obstacle to building models for effective semantic segmentation, and particularly video semantic segmentation, is a lack of large and well annotated datasets. This bottleneck is particularly prohibitive in highly specialized and regulated fields such as medicine and surgery, where video semantic segmentation could have important applications but data and expert annotations are scarce. In these settings, temporal clues and anatomical constraints could be leveraged during training to improve performance. Here, we present Temporally Constrained Neural Networks (TCNN), a semi-supervised framework used for video semantic segmentation of surgical videos. In this work, we show that autoencoder networks can be used to efficiently provide both spatial and temporal supervisory signals to train deep learning models. We test our method on a newly introduced video dataset of laparoscopic cholecystectomy procedures, Endoscapes, and an adaptation of a public dataset of cataract surgeries, CaDIS. We demonstrate that lower-dimensional representations of predicted masks can be leveraged to provide a consistent improvement on both sparsely labeled datasets with no additional computational cost at inference time. Further, the TCNN framework is model-agnostic and can be used in conjunction with other model design choices with minimal additional complexity.

==> tables.tex <==
\begin{table}[]
\caption{Results CaDIS}
% \setlength{\tabcolsep}{3pt}
\begin{tabular}{88mm}[]{cccc}
% \begin{tabular}{|p{25pt}|p{75pt}|p{115pt}|p{25pt}
\hline
Class Name\textbackslash Model & Deeplabv3+ & Deeplabv3+ \& ConvLSTM & Deeplabv3+ \& ConvLSTM \& TCNN \\ \hline
F1 Pupil                        &             &                         &                                \\ \hline
F1 Surgical Tape                &             &                         &                                \\ \hline
F1 Hand                         &             &                         &                                \\ \hline
F1 Eye Retractors               &             &                         &                                \\ \hline
F1 Iris                         &             &                         &                                \\ \hline
F1 Skin                         &             &                         &                                \\ \hline
F1 Cornea                       &             &                         &                                \\ \hline
F1 Instrument                   &             &                         &                                \\ \hline
Mean F1                        &             &                         &                                \\ \hline
Mean IoU                       &             &                         &                                \\ \hline
Mean Pixel Accuracy            &             &                         &                                \\ \hline
\end{tabular}
\end{table}
